On Modal Logics of Connectedness in Metric Spaces

For a positive number a, each metric space carries the relation D_a consisting of those pairs that are of distance less than a apart. A space X is said to be a-connected, if the graph (X,D_a) is connected (that is, there is a D_a-path between every pair of points in X). We give a complete axiomatization of a-connected metric spaces in the language with a family of distance modalities and the universal modality. Then we give a complete axiomatization of the logic of connected (in the classical topological sense) metric spaces in the language with the topological modality, universal modality, and a single distance modality. We also show that these logics have the finite model property.

==> eptcsdata.tex <==
\providecommand{\firstpage}{484}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.27}{10.4204/EPTCS.447.27}}

